Vi(E)va LLM! A Conceptual Stack for Evaluating and Interpreting Generative AI-based Visualizations

The automatic generation of visualizations is an old task that, through the years, has shown more and more interest from the research and practitioner communities. Recently, large language models (LLM) have become an interesting option for supporting generative tasks related to visualization, demonstrating initial promising results. At the same time, several pitfalls, like the multiple ways of instructing an LLM to generate the desired result, the different perspectives leading the generation (code-based, image-based, grammar-based), and the presence of hallucinations even for the visualization generation task, make their usage less affordable than expected. Following similar initiatives for benchmarking LLMs, this paper copes with the problem of modeling the evaluation of a generated visualization through an LLM. We propose a theoretical evaluation stack, EvaLLM, that decomposes the evaluation effort in its atomic components, characterizes their nature, and provides an overview of how to implement and interpret them. We also designed and implemented an evaluation platform that provides a benchmarking resource for the visualization generation task. The platform supports automatic and manual scoring conducted by multiple assessors to support a fine-grained and semantic evaluation based on the EvaLLM stack. Two case studies on GPT3.5-turbo with Code Interpreter and Llama2-70-b models show the benefits of EvaLLM and illustrate interesting results on the current state-of-the-art LLM-generated visualizations.

==> sections/evallm_old.tex <==
\section{EvaLLM: Characterizing the evaluation of LLM-generated visualizations}
\label{sec:stack}

\subsection{Preliminaries}
\label{sec:preliminaries}

In the domain of LLMs applied to visualization generation task (LLM4VIS), the challenge is represented by creating a solution capable of accurately generating a visualization given a dataset $\mathcal{D}$ and a user query $\mathcal{Q}$.
In the forthcoming discussion, it is crucial first to provide a formulation of the problem, as formalized in the following definition:

\begin{mydefinition}{Problem definition}
    Given a tabular dataset $\mathcal{D}$ of $n$ features $\Phi = \{\phi_1,\dots,\phi_n\}$ and a user query $\mathcal{Q}$, an LLM-based visualization recommender system, generates a visualization $V$ that provide the best accuracy concerning $\mathcal{Q}$.
\end{mydefinition}

A task-dependent LLM-VRS should be able to discern and understand the user's intent as conveyed in the input query and generate a visualization that closely aligns with the user's expectations.
Building upon the existing literature for interactive visualizations in this domain, we can categorize the output visualization $\mathcal{V}$ into three classes: image-based visualization, code-based visualization and grammar-based visualization. In the first case, the visualization is directly generated as an image and it represents the only utut of the generation process. In the code-based case, a code snippet is generated and then used to render the visualization. Rendering such output necessitates a specific environment for code execution relative to the language of the generated code. Conversely, the grammar-based case relies on visualization grammars, such as VegaLite, enabling direct rendering by mapping the grammar with one or multiple code environments.
Based on these assumptions, we propose EvaLLM, a conceptual stack that allows the evaluation of all these classes of generated visualizations.

\subsection{Structuring the evaluation: the EvaLLM layers}
\label{se:layers}

EvaLLM is a conceptual stack to model the evaluation for LLM-generated visualization, as shown in Figure~\ref{fig:stack}. Due to the early stage of the LLM models for the visualization field, there is a lack of standard models for assessing the quality of generated visualization, from what their quality depends, or which design elements of a visualization the LLMs are better at accurately generating. Drawing inspiration from the ISO/OSI model~\cite{day1983osi}, EvaLLM involves abstract layers to evaluate specific visualization properties and derive a corresponding quality measure.
From bottom to top, each layer transitions towards a higher level of abstraction. 
%Unlike the ISO/OSI, in EvaLLM the output is a quality measure and does not feed into upper layers. Consequently, each layer operates independently, ensuring autonomy and distinct functionality throughout the evaluation process. 
As illustrated in Figure~\ref{fig:stack}, EvaLLM comprises five primary layers. %, with an optional fifth layer defined as the LLM layer. 
Each layer is subdivided into levels, where the focus is specifically directed towards assessing distinct visualization properties belonging to the same layer. The rationale for this structure is to allows for an initial set of homogeneous categories specialized internally in further detail inside each of them (through levels), and support in this way a fine-grained evaluation of the generated visualization properties, better characterizing the LLMs' expressive power.

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{imgs/stack.pdf}
    \caption{EvaLLMStack: concept evaluation stack for evaluating the LLM-generated visualizations}
    \label{fig:stack}
\end{figure*}

%The image describes the stack depicting the main layers and the levels corresponding to each.
At the base of the EvaLLM stack lies the \textbf{Code layer}, which plays a role in evaluating the fundamental structural properties of a visualization.
The primary question that the Code layer seeks to address is \textit{RQ.1: "Is the visualization consistent within the code environment it is created with?"}. This inquiry delves into the coherence of the visualization within the structure of the related environment (e.g., a generic programming language, a specialized one, or a grammar), checking whether the generated code aligns with the expected structure or evaluating which differences may be present. These differences are mostly syntactical, but they can already present interesting cases that strongly affect the final result quality (i.e., different syntactic structures that give birth to similar visual results, or slightly different codes that produce very different results). In other words, the Code layer focuses on verifying the syntactical correctness and integrity of the visualization's underlying code, laying the groundwork for subsequent layers to delve into more nuanced aspects of evaluation.
Immediately above the Code layer, the evaluation of the visualization is moved to the \textbf{Representation layer}. At this stage, the focus shifts to semantic aspects of the visualization representation, considering the core properties of the visualization with respect to representation rules defined by the literature~\cite{e.g., spence2001information, munzner2009nested}. We distilled from the literature three prominent aspects: the data mapping rules, the choice of the appropriate visual encodings (i.e., marks), and the representation properties of eventual axes or reference visual elements. 
The evaluation question behind this layer is \textit{RQ.2 Are the data representation rules correctly generated in the visualization?}.
We notice that already at this layer it is not granted that some of these aspects are directly captured in the user query (i.e., the query may or may not include a direct reference to these aspects), while they are an integral part of a correct and accurate visualization. For this reason, already at this layer it is needed a more fine-grained and quantitative evaluation with respect to a coarse one based only, for example, on evaluating the correctness of the visual encoding. This evaluation should focus on quantitative distances between the generated content and the expected one.
On top of this layer, there is the \textbf{Presentation layer}. This layer is the third layer in the stack and it assesses the data presentation quality of the visualization from the perceptual standpoint~\cite{ware2019information}. The goal of this layer is to model the design choices for perceptual aspects made by the LLM on the generated visualization to answer the question \textit{RQ.3 Is the visualization correctly presented, comprehensible by a human user, and not presenting perceptual error or illusions hindering the human interpretation of its content?}. For example, it evaluates aspects such as the quality and appropriateness of the color mappings, the distinguishability of visual elements, or the perceptual comprehensibility of the visualized information.
The fourth layer of the stack is the \textbf{Informativeness layer}. It is responsible for measuring the more intrinsic quality of the visualization in terms of its insightfulness and adherence to best practices in visualization literacy, answering the question \textit{RQ.4 Is the visualization insightful, and how well it supports the user in answering its information needs?}. This involves an evaluation that examines the capability of the visualization to convey meaningful insights with respect to the user query and to be aligned with best practices of visualization literacy to ease as much as possible the visualization understanding by the user.
Lastly, the last layer on top of the stack is the \textbf{LLM layer}. 
%It constitutes an optional layer that may be included or omitted within the stack.
The LLM layer contributes twofold at the end of the stack. Its first goal is to evaluate the strategy used to generate the specific visualization. Possible choices relate to single prompting the LLM, applying prompt engineering~\cite{white2023prompt}, or more sophisticated strategies like Chain-of-thought~\cite{wei2022chain}. Evaluate also the configuration elements to discern between different models (i.e., plain foundation model, zero-shot/few-shot approaches, fine-tuning, or a trained-from-scratch new model). In this way, it is possible to evaluate the effort for the generation process on top of the quality of the generated visualization. The second goal is evaluating the visualization by assessing its significance and adherence to best practices in the visualization literature, but this time trying to measure the insightfulness of a visualization with respect to the LLM knowledge and answering the questions \textit{RQ.5 What is the cost of the generated visualization?} and \textit{RQ.6 Is the visualization insightful, based on the LLM knowledge?}. 
%Unlike the application layer, the LLM layer aims to leverage the capabilities of Language Models (LLM) for the evaluation too, through their representation of human knowledge and simulating a human assessment based on the same characteristics. 

%\begin{figure}
%    \centering
%    \includegraphics[width=0.8\linewidth]{imgs/hallucination.pdf}
%    \caption{Visualizaiton hallunication example. In this example, GPT-3.5-turbo correctly predicted the mark type, but it also fabricates a new barchart structure.}
%    \label{fig:hallucincation}
%\end{figure}

==> sections/sota_old.tex <==
\section{Related work}

A Visual Recommendation System (VRS) is an automated system that can generate insightful visualizations from a given dataset. As outlined by in~\cite{podo2023machine}, VRS can be broadly categorized into task-agnostic and task-aware. The former relies solely on the dataset as input, requiring the system to learn how to generate insightful visualizations autonomously. In contrast, the latter involves user guidance through queries or utterances in addition to the dataset, facilitating a more interactive and user-informed approach to data visualization.
This section delves into the contributions coping with task-aware VRSs, offering a comprehensive overview of how methods based on Large Language Models (LLMs) are employed and the potential enhancements they could bring. Furthermore, we explore also more classic approaches, including rule-based and machine-learning methods~\cite{setlur2016eviza, luo2021natural, srinivasan2023bolt, kim2021data, narechania2020nl4dv, song2022rgvisnet, gao2015datatone}. Discussing these non-LLM-based techniques provides a broader context for the landscape of VRS methodologies.
Finally, the section addresses existing research investigating the quality and capabilities of an LLM-based Visual Recommendation System (LLM-VRS). It adopts an empirical approach to evaluate these models, specifically in the visualization generation task(s) context.
In the rest of the paper, we classify traditional approaches as a broader category encompassing rule-based, machine learning, and deep learning methods. In contrast, we use the term ``LLM-based'' to refer specifically to methods involving only Large Language Models. This distinction allows for a more precise delineation and understanding of the different classes of approaches in the VRS domain.

\subsection{VRS task-aware benchmarks}
As discussed, the task-aware VRSs require user utterance along with the dataset as input. 
%This implies the need for benchmarks, including the data-visualization pairs and the dataset in input. These benchmarks are crucial for both the training of such models and for the evaluation and comparative analysis studies.
To assess a model's performance on the given task, several datasets are available, each with its unique characteristics:
nvBench dataset~\cite{luo2021nvbench} presents 25,750 triplets (data, utterance, chart) sourced from 105 domains of tabular data. Despite its comprehensive nature, it is worth noting that many utterances in the nvBench dataset provide explicit visualization specifications, including explicit details about the expected visualization, like the data columns, the chart type or other visualization properties. For instance, the following example: ``A pie chart showing the number of faculty members for each rank.'' precisely communicates the user's visualization expectations regarding the chart type. Moreover it covers only the most frequent visualization types, such as: bar, pie, line, scatter, stacked bar, grouping line, and grouping scatter.
The NLVCorpus~\cite{srinivasan2021collecting} comprises 893 utterances related to ten types of charts. However, the NLVCorpus is constrained by its reliance on only three data tables.
In the work by Tian et al.~\cite{tian2023chartgpt}, a new dataset is proposed based on the nvBench dataset. The authors curate this new dataset by initially selecting utterances involving only one data table, eliminating pairs requiring multiple tables. They then employ GPT-3 to abstract the utterances, thereby reducing explicitness. While this dataset stands as an essential resource in the field, it is important to note that it relies on synthetic pairs.
Quda~\cite{fu2020quda} encompasses 14,035 user utterance queries spanning various analytical tasks. However, it lacks associated charts, which limits its utility for visualization evaluation scenarios.
%MIT-VisText~\cite{2023-vistext} puts forward a dataset of 12,441 pairs of charts and captions that describe the charts’ construction, report key statistics, and identify perceptual and cognitive phenomena. The dataset being a bit different form others, it provides scene-graphs that are a high-level rich description of the data and values which can be processed and shaped into a structured prompt for the LLM to generate a visualization. It also provides Vega-Lite specifications which can be considered for visualization comparison metrics also.
This diversity in datasets provides researchers with options for evaluating models, each dataset bringing its strengths and limitations. At the same time, none copes with the problem of defining a granular set of metrics and elements to consider for comparing the tested approaches. 

\subsection{Traditional visualization generation methods}
In the literature, the task-aware VRS models predominantly rely on traditional methodologies.
For example, in ~\cite{setlur2016eviza} the authors introduce an interactive visualization tool that employs a hybrid approach integrating Natural Language Processing (NLP) and decision rules. This system combines a probabilistic grammar approach with predefined rules that can be dynamically updated based on the underlying data. This approach offers the advantage of reduced computational complexity compared to machine/deep learning methods, resulting in a faster interaction. 
%The emphasis on computational efficiency is a crucial strength of this approach.
In ~\cite{srinivasan2023bolt}, the authors present BOLT, a web-based platform for multi-dashboard authoring using natural language. The authors propose a system based on traditional NLP techniques to map user utterances to prevalent dashboard objectives and generate appropriate visualizations. 
The novelty of this paper lies in the focus on higher dashboard objectives that focus on the overall problem the user is trying to solve (e.g., change analysis) rather than lower ones that involve simpler visualization operations (e.g., sorting). Although user validation demonstrates the positive impact of natural language on interaction, the inherent challenge of handling ambiguous user utterances persists, posing difficulties for classical NLP methods.
In contrast, ~\cite{narechania2020nl4dv} introduce a method for interacting with a dataset based on NLP, focusing on generating a single visualization rather than suggesting a complete dashboard. The emphasis here is on providing tailored visualizations through NLP techniques.
Moving beyond rule-based approaches, ~\cite{luo2021natural} propose ncNet, a seq2seq model that translates Natural Language Queries (NLQs) into a custom visualization grammar, Vega-Zero. This transformer-based encoder-decoder architecture employs an attention-forcing method and is trained on the nvBench dataset. While ncNet represents a breakthrough in processing the user inputs as free-text, it still faces challenges in handling ambiguous and ill-posed natural queries.
To address these limitations, ~\cite{song2022rgvisnet} introduced RGVisNet, a retrieval and generation-based approach. Instead of directly translating NLQs into the visualization grammar, the network is divided into two components: (i) a data visualizations query retrieval network and (ii) a data visualizations query revision network. The retrieval network, based on a Graph Neural Network (GNN), retrieves relevant data visualizations from a database, while the revision network adjusts the candidate based on the expected data visualization outcomes through a decoder structure.

Despite the effectiveness of these non-LLM-based systems, they grapple with the challenge of capturing underlying semantics in user utterances, mainly when dealing with ambiguous expressions. This may not lead to a ideal generated visualization as a result.

\subsection{LLM-based visualization generation methods}
As discussed, the rise of the LLMs has posed new research questions in different fields, including the data visualization field. New approaches have been proposed in this direction. 
%Dibia et al.~\cite{dibia2023lida} introduces a novel methodology for implementing a Visual Recommendation System (VRS) leveraging the capabilities of Large Language Models (LLMs). This work explores new frontiers in automated visualization generation by harnessing the potential LLMs offer. They also propose a system, LIDA, as a modular pipeline with four modules, the first three of which employ GPT-4~\cite{openai2023gpt}.
%The initial module, the \textit{Summarizer}, extracts meaningful information from the data and converts it into a rich text description. The \textit{Goals Generation} module identifies the most suitable visualization goals based on the dataset description. Subsequently, the \textit{Code Generator} module utilizes the extracted description and goals to generate the code for the visualizations. The final module, a non-LLM-based component, enhances the final design of the visualization.
%To shape the output of each phase, prompt engineering techniques~\cite{white2023prompt} are applied without altering the underlying architecture of the model. We complement this approach as we are focused on evaluating the final result and allow fine-grained evaluation of generated visualization more than providing novel ways to generate them. 
% Unlike the previous contribution, which demonstrates how an LLM can be involved in task-agnostic LLM-based VRS, 
In \cite{hong2023conversational}, the authors propose AI Thread, a chatbot for multi-threaded analytic conversations. Using the chain-of-thoughts reasoning technique \cite{wei2022chain}, the system leverages GPT-3.5 capabilities in Python to map the user utterance into a visualization using Matplot and Seaborn libraries. Moreover, the tool proposes a two-view interface: the main chat, that is, the chat view interaction, and the thread panel that allows for edits on the visualizations in the main board. A different approach is proposed in \cite{chen2022nl2interface}. The authors discuss a method based on few-shot learning~\cite{wang2020generalizing} at inference time on the Codex LLM model by OpenAI~\cite{finnie2022robots}. The model is fed with natural language-SQL (NL2SQL) pairs examples and the user's natural language query to aid in task understanding. The result is then converted into Vega-Lite specifications using a rule-based approach~\cite{chen2022pi2}. The authors emphasize that their approach can achieve valuable results without requiring model tuning . However, the study's evaluation is conducted on a limited number of examples without providing any findings about the quality of the explored samples, raising questions about the generalizability of the approach.
Similarly, Maddigan et al.~\cite{maddigan2023chat2vis} present a comparable study involving Codex, GPT -3, and ChatGPT. Like the previous work, the study lacks a comprehensive discussion of results and relies on a small number of evaluation samples. 
%leaving room for a more extensive assessment.
Finally, Tian et al.~\cite{tian2023chartgpt} recently introduced ChartGPT, a multi-step pipeline incorporating LLMs into various stages, breaking down the visualization generation problem into logical steps. The authors fine-tune FLAN-t5~\cite{chung2022scaling} to align the model with the intended task. The evaluation is extensive in the number of tests but is still executed using a custom evaluation scheme. This problem is common even to other papers presented in this section, leading us to study deeply how a general framework could support LLM-generated visualizations.

\subsection{Evaluating LLMs visualizations}
Despite the impressive performances demonstrated by these new approaches, there needs to be more evaluation approaches and standard methodologies to assess the understating capabilities in the data visualization domain. To fill this gap, some researchers have started to map these capabilities, proposing evaluation methods. 
For example, in \cite{chen2023beyond} present an evaluation study focusing on GPT-3.4 and GPT-4, examining these models beyond the conventional visualization generation task considered from just the code generation perspective. Instead, the study delves into multiple facets, such as data interpretation, visualization design, visual data exploration support, and insight communication. To assess the model's proficiency, they tasked GPT with completing various quizzes and producing visualizations based on the data visualization course of Harvard CS171. GPT was asked to perform random tasks from the dataset, including quizzes and homework, and a group of fellows evaluated the results. This study introduces an initial evaluation approach to understand how well GPT can address challenges closely tied to visualization tasks. While using general categories of elements considered during a visualization evaluation, the work focuses more on their application than the conceptual modeling of what it means to evaluate an LLM-generated visualization. It also presents interesting considerations on this topic, and we took inspiration from them to define our evaluation conceptual stack.
Another in-depth study is conducted by Kim et al.~\cite{kim2023good}, where the authors thoroughly explore the capabilities and limitations of ChatGPT in visualization tasks. They pose a series of questions from the VisGuides forum and compare the answers with human responses from the original questions on the blog. The study observes that ChatGPT performs similarly to human responses and, in some cases, even outperforms them. The authors then asked a group of data visualization experts to evaluate visualizations provided by both ChatGPT and domain experts without revealing the source. The study concludes that users prefer human feedback over LLM feedback, highlighting the main disadvantages of ChatGPT's lack of discussion and emphasizing the potential advantage of a design knowledge agent. We identified similar needs in including human assessment even for LLM-based visualizations, which informed the creation of EvaLLM.
Finally, Tao et al.~\cite{tao2023mapping} investigate ChatGPT's capability to generate abstract maps through two main experiments. The first experiment assesses the model's ability to generate thematic maps based on specified map styles and data sources in the prompts. The second experiment involves generating mental maps from the data. The study concludes that ChatGPT can assist in generating maps and enhance productivity. However, it notes the model's dependence on external tools for visualization generation and difficulty achieving the desired output.
While these works contribute to integrating LLMs into existing data visualization pipelines, few have systematically studied the main characteristics needed to evaluate a generated visualization and how to organize and leverage them to benchmark automatic generators, creating a taxonomy of recurring errors. 
%Furthermore, none have proposed a comprehensive evaluation process to quantitatively and qualitatively compare model results with the expected ground truth. 
To fill this gap, this paper proposes a conceptual stack that includes both automatic quantitative metrics and human-based evaluation metrics and investigates its application to LLM-based visualizations.

%Per ogni related, introdurre cosa fa e come si differenzia da noi. Alcuni si somigliano e si raggruppano, decrivendo come si specializzano e come noi ci differenziamo

